Learning Symbolic Rules over Abstract Meaning Representations for Textual Reinforcement Learning

Text-based reinforcement learning agents have predominantly been neural network-based models with embeddings-based representation, learning uninterpretable policies that often do not generalize well to unseen games. On the other hand, neuro-symbolic methods, specifically those that leverage an intermediate formal representation, are gaining significant attention in language understanding tasks. This is because of their advantages ranging from inherent interpretability, the lesser requirement of training data, and being generalizable in scenarios with unseen data. Therefore, in this paper, we propose a modular, NEuro-Symbolic Textual Agent (NESTA) that combines a generic semantic parser with a rule induction system to learn abstract interpretable rules as policies. Our experiments on established text-based game benchmarks show that the proposed NESTA method outperforms deep reinforcement learning-based techniques by achieving better generalization to unseen test games and learning from fewer training interactions.

==> sections/introduction.tex <==
\section{Introduction}

 \begin{figure}[tb]
		\centering
        % \includegraphics[width=0.9\linewidth]{figures/intro.pdf}
        \includegraphics[width=1.00\linewidth]{figures/front_page.png}
		\caption{Our proposed NESTA model learns interpretable actions rules as policy using ILP and outperforms SOTA deep RL methods on TWC hard games.}
		\label{fig:front_page}
		\vspace{-3mm}
\end{figure}

 Text-based games (TBGs)~\cite{cote2018textworld} serve as a popular test-bench for quasi real-world interactive setting. TBGs involve obtaining a textual representation of the observation text which is then used for issuing an action command. Since TBGs are typically in the partial observation setting, the action commands allow the agent to explore unobserved parts of the environment. The agent's goal is to reach a particular goal which is learned from a reward signal from the environment. Deep reinforcement learning methods are increasingly being used for such text-based reinforcement learning (RL) problems. Most approaches~\cite{narasimhan-etal-2015-language,adolphs2019ledeepchef,he-etal-2016-deep-reinforcement, yuan2019counting} use the surface text form of the observations to learn action policies that give an output probability distribution over the action commands. However, such policies do not generalize well to unseen test cases because they overfit the training examples.%, especially in low-data training settings.

 Graph-based methods~\cite{ammanabrolu2018playing, ammanabrolu2020graph, adhikari2020learning, murugesan2021efficient} extracts graphical representations~\cite{angeli2015leveraging} from the textual observations. This class of methods hypothesizes that learning a policy on structured representations can lead to a stronger generalization and they show better performance on test games compared to the surface text embedding-based policies. Recent neuro-symbolic RL methods~\cite{chaudhury2021neuro, kimura2021neuro} show close to perfect performance on simple hand-crafted textworld settings. However, these methods use domain-specific predicate design that is unlikely to generalize to TBGs with complex goal settings.
 
To address the issues of poor generalization and sample efficiency, we present a neuro-symbolic textual agent (NESTA) that learns first-order horn clauses as action rules from symbolic observation representations. We hypothesize that an ideal policy for solving TBGs requires learning abstract action rules that can reason over entities that it has not seen in training. Therefore, our method learns abstract rules over symbolic facts obtained from observation text at each step. Our symbolic fact extraction uses Abstract Meaning Representations (AMR) of the surface text that use generic domain-agnostic predicates from Propbank~\cite{palmer2005proposition} and unlike previous methods NESTA does not require hand-crafted domain-specific predicate design. NESTA learns the symbolic observation facts at each step are used to perform rule induction for learning action rules based on the expected reward maximization loss. We use Inductive Logic Programming (ILP)~\cite{muggleton1996learning} for learning first-order lifted rules and hence can generalize better to entities unseen during training. 

Our empirical analysis on commonsense-aware textworld games shows that our neuro-symbolic methods outperform deep RL methods while learning from lesser training interactions and producing human interpretable rules. Figure~\ref{fig:front_page} illustrates the overview of our NESTA method and reports that our method outperforms the SOTA method on two widely used metrics. Our main contributions in this work are: (1) We propose a neuro-symbolic agent for learning action probabilities instead of using a black-box neural network policy and show that it generalizes better than traditional deep TBRL methods, (2) Proposed NESTA has better sample efficiency compared to traditional text-based RL obtaining better test performance from almost $0.5\times$ lesser training interactions, and (3) Our method produces human interpretable rules that can be easily debugged by humans-in-the-loop correction.


\begin{figure*}[tb]
		\centering
        % \includegraphics[width=0.9\linewidth]{figures/intro.pdf}
        \includegraphics[width=0.99\linewidth]{figures/intro_new.png}
		\caption{Overview of our method for neuro-symbolic reasoning. Our methods first extract symbolic facts from the surface text observations. During training, NESTA learns first-order lifted rules based on the reward signals. The learned rules are then used for sampling the action commands for producing the episodic trajectory.}
		\label{fig:method}
		\vspace{-3mm}
\end{figure*}

==> sections/prelim.tex <==
\section{Preliminaries}
\subsection{Text-based Games}
